Energy Communities: From European Law to Numerical Modeling

In 2019, the European Union introduced two new actors in the European energy system: Renewable and Citizen Energy Communities (RECs and CECs). Modelling these two new actors and their effects on the energy system is crucial when implementing the European Legislation, incorporating energy communities (ECs) into the electric grid, planning ECs, and conducting academic research. This paper aims to bridge the gap between the letter of the law and numerical models of ECs. After introducing RECs and CECs, we list elements of the law to be considered by regulators, distribution system operators, EC planners, researchers, and other stakeholders when modelling ECs. Finally, we provide three case studies of EC models that explicitly include elements of the European Law.

==> EEM2020_arxiv version/Data/data.tex <==





==> EEM2020_arxiv version/Figures/fig_key_rep.tex <==
\begin{figure}
\centering
\begin{tikzpicture}

\begin{axis}[
       cycle list/Accent,
  date coordinates in=x,
  ticklabel style = {font=\footnotesize},
  xticklabel=\hour,
  xmin  = 00-01-00 04:00, xmax = 00-01-00 19:00,
  width=.95\linewidth, height=4cm, 
  y label style={ font=\footnotesize},
    x label style={font=\footnotesize},
	ylabel=load (kW), xlabel= time (hour),
		legend style={at={(0.05,0.85)}, draw=none,fill=none,
		anchor=west,legend columns=1, font=\footnotesize},
]
\path[name path=axis] (axis cs:00-01-00 00:00,0) -- (axis cs:00-01-00 23:30,0);
\addplot[const plot,name path=LOAD, color=blue, thick] table [x=time,y=load, col sep=comma] {actual_key_sample.dat};
\addplot[const plot, name path=SOLAR, color=orange, line width=0pt,forget plot] table [x=time,y=production, col sep=comma] {actual_key_sample.dat};
\addplot[const plot,name path=B, color=black, line width=0pt,forget plot] table [x=time,y =x1 , col sep=comma] {actual_key_sample.dat};
\addplot[const plot,name path=C, color=black, line width=0pt,forget plot] table [x=time,y =x2 , col sep=comma] {actual_key_sample.dat};
\addplot[const plot,name path=D, color=black, line width=0pt,forget plot] table [x=time,y =x3 , col sep=comma] {actual_key_sample.dat};
\addplot[const plot,name path=E, color=black, line width=0pt,forget plot] table [x=time,y =x4 , col sep=comma] {actual_key_sample.dat};
\addplot[const plot,name path=F, color=black, line width=0pt,forget plot] table [x=time,y =x5 , col sep=comma] {actual_key_sample.dat};
\addplot[const plot,name path=G, color=black, line width=0pt,forget plot] table [x=time,y =x6 , col sep=comma] {actual_key_sample.dat};
\addplot[const plot,name path=H, color=black, line width=0pt,forget plot] table [x=time,y =x7 , col sep=comma] {actual_key_sample.dat};
\addplot[const plot,name path=I, color=black, line width=0pt,forget plot] table [x=time,y =x8 , col sep=comma] {actual_key_sample.dat};
\addplot[const plot,name path=J, color=black, line width=0pt,forget plot] table [x=time,y =x9 , col sep=comma] {actual_key_sample.dat};
\addplot[const plot,name path=K, color=black, line width=0pt,forget plot] table [x=time,y =x10 , col sep=comma] {actual_key_sample.dat};
\addplot[const plot,name path=L, color=black, line width=0pt,forget plot] table [x=time,y =x11 , col sep=comma] {actual_key_sample.dat};
\addplot[const plot,name path=M, color=black, line width=0pt,forget plot] table [x=time,y =x12 , col sep=comma] {actual_key_sample.dat};
\addplot[const plot,name path=N, color=black, line width=0pt,forget plot] table [x=time,y =x13 , col sep=comma] {actual_key_sample.dat};
\addplot[const plot,name path=O, color=black, line width=0pt,forget plot] table [x=time,y =x14 , col sep=comma] {actual_key_sample.dat};
\addplot[const plot,name path=P, color=black, line width=0pt,forget plot] table [x=time,y =x15 , col sep=comma] {actual_key_sample.dat};
\addplot[color=orange] fill between[of=P and SOLAR];
%\path[name path=B] table [x=time,y = x1  , col sep=comma] {actual_key_sample.dat};
\addplot fill between[of=B and axis,forget plot];
\addplot fill between[of=C and B,forget plot];
\addplot fill between[of=D and C,forget plot];
\addplot fill between[of=E and D,forget plot];
\addplot fill between[of=F and E,forget plot];
\addplot fill between[of=G and F,forget plot];
\addplot fill between[of=H and G,forget plot];
\addplot fill between[of=I and H,forget plot];
\addplot fill between[of=J and I,forget plot];
\addplot fill between[of=K and J,forget plot];
\addplot fill between[of=L and K,forget plot];
\addplot fill between[of=M and L,forget plot];
\addplot fill between[of=N and M,forget plot];
\addplot fill between[of=O and N,forget plot];
\addplot fill between[of=P and O,forget plot];
\legend{total load, surplus}

\node[anchor=south] (source) at (axis cs:00-01-00 15:30, 20){\footnotesize repartitioned energy};
       \node (destination) at (axis cs: 00-01-00 12:15,5){};
       \draw[->, thick](source)--(destination);
\end{axis}

\end{tikzpicture}

  \caption{Total load, the key of repartition, and surplus for a sample day. The repartitioned energy is represented by the colored area under the blue curve with each color representing a different community member.}
  \label{fig:key_example}
\end{figure}

==> EEM2020_arxiv version/Figures/fig_mechelen_EC.tex <==
\begin{figure}
\centering

\includegraphics[width=0.5\textwidth]{Figures/EC_Wallonia.png}

  \caption{The PROSUMER EC model distinguishes from individual self-consumption, collective self-consumption, and consumption from the grid. These distinctions are important to calculate the financial impact that different tariff and tax designs can have on the different stakeholders related to an EC (participants, the community as a whole, the DSO and the traditional energy supplier).}
  \label{fig:EC_mechelen}
\end{figure}
